Personalized Re-ranking for Recommendation

Ranking is a core task in recommender systems, which aims at providing an ordered list of items to users. Typically, a ranking function is learned from the labeled dataset to optimize the global performance, which produces a ranking score for each individual item. However, it may be sub-optimal because the scoring function applies to each item individually and does not explicitly consider the mutual influence between items, as well as the differences of users' preferences or intents. Therefore, we propose a personalized re-ranking model for recommender systems. The proposed re-ranking model can be easily deployed as a follow-up modular after any ranking algorithm, by directly using the existing ranking feature vectors. It directly optimizes the whole recommendation list by employing a transformer structure to efficiently encode the information of all items in the list. Specifically, the Transformer applies a self-attention mechanism that directly models the global relationships between any pair of items in the whole list. We confirm that the performance can be further improved by introducing pre-trained embedding to learn personalized encoding functions for different users. Experimental results on both offline benchmarks and real-world online e-commerce systems demonstrate the significant improvements of the proposed re-ranking model.

==> em1_fig.tex <==
% transformer 局部放大？
\tikzset{
  item/.style = {draw, rectangle, fill=cosmic_latte, minimum width=3cm, minimum height=0.5cm},
  relu/.style = {draw, rectangle, fill=cosmic_latte, minimum width=7cm, minimum height=0.5cm},
  relu2/.style = {draw, rectangle, fill=blue2, minimum width=5cm, minimum height=0.5cm},
  sigmoid/.style = {draw, rectangle, fill=cosmic_latte, minimum width=3cm, minimum height=0.5cm},
  pvector/.style = {draw, rectangle, dashed, fill=blue2, minimum width=2.8em, minimum height=1.8em},
}


%portafino

\begin{figure}[tb]
\centering
\begin{tikzpicture}[]

% 两个embedding向量
\node[item] (e1) at (0, 0) {click vector};
\node[item, right of=e1, node distance=3cm] (e2) {item embedding};
\node[item, right of=e2, node distance=3cm] (e3) {user side information};

\node[relu, above of=e2, node distance=1cm] (e4) {Layer$_1$};
\node[above of=e4, node distance=0.7cm] (e0) {$\vdots$};
\node[relu2, above of=e0, node distance=0.5cm] (e5) {Layer$_n$};
\node[sigmoid, above of=e5, node distance=1cm] (e6) {sigmoid};

\node[pvector, right of=e6, node distance=4cm] (pv) {$\mathbf{PV}_{i_n}$};
% 箭头
\draw [->,thick,dotted] (e5.east) to [in = -100, out = 0] (pv.south);

\node[below of=e1, node distance=1cm] (input1) {user's click history $\mathcal{H}(u)$ };
\node[below of=e2, node distance=1cm] (input2) {target item $i_n$};
\node[below of=e3, node distance=1cm] (input3) {\{user id, gender, age, $\cdots$\}};

\node[above of=e6, node distance=1cm] (output) {$P(y_{i_n}|\theta^{'},\mathcal{H}_u, u)$};


% 下面的箭头
\draw[-{Latex[length=1mm, width=0.8mm]}] ($(input1.north)$) -- ($(e1.south)$) ;
\draw[-{Latex[length=1mm, width=0.8mm]}] ($(input2.north)$) -- ($(e2.south)$) ;
\draw[-{Latex[length=1mm, width=0.8mm]}] ($(input3.north)$) -- ($(e3.south)$) ;

\draw[-{Latex[length=1mm, width=0.8mm]}] ($(e2.north)$) -- ($(e4.south)$) ;
\draw[-{Latex[length=1mm, width=0.8mm]}] ($(e5.north)$) -- ($(e6.south)$) ;
\draw[-{Latex[length=1mm, width=0.8mm]}] ($(e6.north)$) -- ($(output.south)$) ;


\end{tikzpicture}
    \caption{The model structure of pre-trained model. $P(y_{i_n}|\theta^{'},\mathcal{H}_u, u)$ is the predicted probability whether the item $i_n$ will be clicked by user $u$. $\mathcal{H}(u)=[i_{n-k}, ... , i_{n-2}, i_{n-1}]$ is the sequence of items clicked by the user $u$. $\mathbf{PV}_{i_n}$ is the personalized vector of user $u$ on item $i_n$.}
    \label{fig:pv}
\end{figure}
